AMoPO: Adaptive Multi-objective Preference Optimization without Reward Models and Reference Models

Existing multi-objective preference alignment methods for large language models (LLMs) face limitations: (1) the inability to effectively balance various preference dimensions, and (2) reliance on auxiliary reward/reference models introduces computational complexity. To address these challenges, we propose Adaptive Multi-objective Preference Optimization (AMoPO), a novel framework that achieves dynamic balance across preference dimensions. By introducing the multi-objective optimization paradigm to use the dimension-aware generation metrics as implicit rewards, AMoPO aligns LLMs with diverse preferences without additional reward models or reference models. We introduce an adaptive weight assignment mechanism that models the generation space as a Gaussian distribution, allowing dynamic prioritization of preference dimensions. Empirical results demonstrate that AMoPO outperforms state-of-the-art baselines by 28.5%, and the experiments on 7B, 14B, and 32B models reveal the scaling ability of AMoPO. Moreover, additional analysis of multiple dimensions verifies its adaptability and effectiveness. These findings validate AMoPO's capability to achieve dimension-aware preference alignment, highlighting its superiority. Our codes and datasets are available at https://github.com/Javkonline/AMoPO.

==> latex/images/main/amopo_alg_2.tex <==
\begin{algorithm*}

\caption{AMoPO}
\label{alg:amopo}
\setstretch{0.5}
\KwIn{Policy model $\pi_\theta$, Multiple objective $\bm{d}$, Mapping function $f$, Number epochs $epochs$, Coefficient $\beta$, Learning rate $\eta$}
\KwIn{Dataset $\mathcal{D} = \{ (x, {y_w}, {y_l}, score)^i\}_{i=1}^{N}$ of samples size $N$ with different dimension scores.}
\For{epoch in range($epochs$)}{
    {\textbf{Initialize:} All tokens probabilities $\bm{p}= [\;]$, Weights $\bm\alpha=[\;]$, Multiple loss $\bm{\mathcal{L}} = [\;]$}\\
    Sample a batch $\mathcal{D}_s = \{ (x, {y_w}, {y_l}, score)^s\}_{s=1}^{S}$ from $\mathcal{D}$;\\
    
    \For{$d$ in $\bm{d}$}{
        Use the dimension $d$ and the mapping function $f$ to get the unique prompt template $x^* = f(x|d)$;\\
        Merge all samples $\mathcal{D}_j^d = \{ (x^*, {y_w},{y_l}, score_d)^s\}_{s=1}^{S} $; \\
        Predict the all tokens probabilities $p_d^{w}={\{<t_i^w,p_i^w>\}}_{i=1}^{|y_w|}$ and $p_d^{l}={\{<t_i^l,p_i^l>\}}_{i=1}^{|y_l|}$ based on $\pi_\theta(y_w|x^*)$ and $\pi_\theta(y_l|x^*)$;\\
        Calculate the sum probabilities $p_d = p_d^w+p_d^l$;\\
        Model $p_d$ based on Gaussian Sample to get the weight $\alpha_d$;\\
        Calculate current function $l=\log\sigma(\frac{\beta}{|{y_w}|} \log \pi_\theta({y_w} \mid x^{*})-\frac{\beta}{|{y_l}|} \log \pi_\theta({y_l} \mid x^{*}))$;\\
        $\bm{p} \gets p_d$ ;
        $\bm\alpha \gets \alpha_d$
        $\bm{\mathcal{L}} \gets l$;\\
    }
    Normalize different dimensions weights $\bm{\alpha}$ by Eq.\eqref{Eq.7};\\
    $\theta \gets \theta+\eta{\nabla_\theta}\mathbb{E}_{(x, y_w, y_l,score)\sim \mathcal{D}_s} \bm{\alpha}^{T}\bm{\mathcal{L}}  $
}
\KwOut{$\pi_\theta$}
\end{algorithm*}
\end{algorithm*}


==> latex/sections_article/1_introduction.tex <==

Large Language Models (LLMs), pre-trained on a large-scale corpus, have demonstrated remarkable capabilities on various upstream and downstream tasks across different domains, such as question answering~\cite{} and information extraction~\cite{MIE2024xu}. However, due to the disorganized and chaotic nature of the training corpus, it becomes crucial to align large language models with human values and intentions. 
Reinforcement learning from human feedback (RLHF)~\cite{ChristianoDRLHP2017} is a popular method to achieve alignment in the process of fine-tuning LLMs. While RLHF has achieved impressive results, it involves training the reward function and integrating this reward function into the reinforcement learning training process, issues such as training instability and reward collapse may arise. In contrast, Direct Preference Optimization (DPO)~\cite{DPO2023Rafailov} is a simpler algorithm, which directly optimize a language model without explicit reward model to align human preferences.

While the considerable success has already been achieved in aligning with human preferences, it is unrealistic to reflect true human preferences through a single dimension~\cite{helpsteer22024wang, ultrafeedback2024cui, rewardsoup2023Rame}.
Therefore, numerous researchers have focused on aligning with human preferences by considering multi-dimensional evaluation metrics.
Multi-objective RLHF (MORLHF)~\cite{fintunerlhf2024wu} come into being, which divide human preference into few dimensions~\cite{rewardsoup2023Rame}, e.g.,helpfulness, correctness, and then train a set of different reward models for candidate language models using reinforcement learning. 
Similar to RLHF, MORLHF is more complex and the significant computational overhead associated with the training of reward models and language models.
To alleviate the computational overhead, MODPO~\cite{MODPO2024zhou} introduce an RL-free method by extending DPO for multiple alignment objectives. 
MODPO classifies various dimensions into two distinct sets: one for conducting preference optimization training using DPO, and the other for training a reward model. The reward scores from the preference-optimized dimension are subsequently integrated into the MODPO loss function as a margin. 
Subsequently, by assigning different weights to these dimensions, we calculate the cumulative reward for the MODPO training process.

However, MODPO interprets additional dimensions is entirely dependent on the formulation of the reward model. Training a complex and comprehensive reward model is often costly. 
Besides, MODPO is based DPO, which also not directly aligned with the metric used for generation and need more computing resources to employ reference model. 
Furthermore, these multi-objective methods are using fixed weights to train their models, which greatly influenced the scalability of the model.

In this work, we propose Reference-free Multi-objective Preference Optimization (\ourtitle), a simple yet effective multi-objective preference optimization algorithm. 
We incorporate the generation metrics of language models as the implicit rewards and design distinct templates for different dimensions, enabling the language model to autonomously learn the meanings associated with each dimension.
Additionally, language models can automate the assignment of weights between dimensions based on the current output space.
In summary, our~\ourtitle~has the following properties:

\begin{itemize}
    \item \textbf{Low power consumption:}~\ourtitle~does not require any other reward model and reference model, which make it more lightweight and efficient compared to other multi-objective preference optimization methods, as we utilize a multi-dimensional generation metric~\cite{simpo2024meng} as the implicit reward function. This approach allows the language model to genuinely enhance its capability for multi-dimensional generation.
    
    \item \textbf{Automated weighted assignment:} Unlike fixed weighted assignment,~\ourtitle~employs Gaussian sampling to model the probabilities of all tokens in the generative space of the current dimension according to the language model. The results of the Gaussian sampling are then used to adaptively allocate weights to the current dimension.

    \item \textbf{Performance:}~\ourtitle~significantly outperforms DPO, SimPO, MODPO and their latest variants (e.g., ORPO, Cal-DPO).~\ourtitle~achieves state-of-the-art (SOTA) results on three public benchmark, including AlpacaEval 2, Arena-Hard and MT-bench. It achieves up to a 5.3 point improvement on AlpacaEval 2, a 4.6 point improvement on Arena-Hard and a 0.1 rating improvement on MT-bench.
\end{itemize}








==> latex/sections_article/2_related_work.tex <==


\subsection{Direct Preference Optimization}
While Large Language Models (LLMs) can learn board world knowledge, precisely aligning with human preferences remains a challenging issue. Compared with the commonly used reinforcement learning from (or AI) human feedback (RLHF/RLAHF)~\cite{ChristianoDRLHP2017}, DPO~\cite{DPO2023Rafailov} eliminates the need for training a complex reward model, offering a more stable and efficient alignment scheme.

% Based on DPO, ORPO~\cite{ORPO2024Hong} simplifies training
% with odds ratio-based penalties. Unlike ORPO, Cal-DPO~\cite{caldpo2024xiao} does not directly enhance the reward margin between winning and losing responses. Instead, it introduces an additional hyperparameter that boosts the reward for generating winning responses while reducing the reward for generating losing responses.
Based on DPO, numerous variants of preference optimization have emerged.
ORPO~\cite{ORPO2024Hong} simplifies training with odds ratio-based penalties and jointly trains with SFT objective.
R-DPO~\cite{rdpo2024Park} increases the margin in the DPO stage by introducing regularization on the length of the policy model responses.
Unlike R-DPO, Cal-DPO~\cite{caldpo2024xiao} does not directly enhance the reward margin between winning and losing responses. Instead, it introduces an additional hyperparameter that boosts the reward for generating winning responses while reducing the reward for generating losing responses.
IPO~\cite{ipo2024Azar} uses pointwise rewards to avoid DPO's assumption.


\subsection{Reference-Free Reward Preference Optimization}
The preference alignment based on DPO has a significant characteristic, which is the requirement of a reference model to control the KL divergence between the optimized model and the reference model. However, this approach not only requires additional memory to deploy the reference model during training, but also presents a gap between the reward metrics during training and the actual model generation metrics. To tackle this, the CPO~\cite{CPO2024xu} demonstrates that the loss of DPO can be effectively approximated using a unified reference model.
SimPO~\cite{simpo2024meng} replaces the reward in DPO with a sequence generated by the policy model that approximates the maximization of the mean log-likelihood, which serves as the new reward.


\subsection{Multi-objective Preference Optimization}

Despite the increasing number of variations in preference optimization~\cite{ipo2024Azar, KTO2024Ethayarajh}, the human preferences are intrinsically diverse. Single-dimensional optimization is inadequate in capturing this diversity because current preference optimization data only represents average preferences. Consequently, numerous researchers have concentrated on the development of multi-dimensional preference datasets, such as HelpSteer~\cite{helpsteer2024wang}, HelpSteer2~\cite{helpsteer22024wang}, and UltraFeedback~\cite{ultrafeedback2024cui}. These datasets entail the decomposition of responses to prompts into several dimensions, including helpfulness, instruction following and so on. This has stimulated extensive investigations into multidimensional preference optimization. MODPO~\cite{MODPO2024zhou} is an extension of DPO. MODPO segments the training procedure into two distinct phases. Initially, it trains the reward model on dimensions excluding the preference optimization dimension. Subsequently, it integrates the scores obtained from the reward model for the current dimension into the preference optimization training process.


==> latex/sections_article/3_preliminary.tex <==
% Preliminary

\textbf{Multi-objective Preference Dataset. }A single-dimensional preference dataset can be defined as $\mathcal{D} = \{ x^{(i)}, {y_w}^{(i)}, {y_l}^{(i)}\}_{i=1}^{N}$, where $x^{(i)}$, ${y_w}^{(i)}$ and ${y_l}^{(i)}$ denote instruction, winning response and losing response, respectively. Comparing with single-dimensional preference dataset, multi-objective preference dataset not only contains basic preference objective (i.e., winning response and losing response), but also has multi-dimensional scores for each response.
It can be formulated as $\bm{\mathcal{D}} = [ \mathcal{D}_1, \mathcal{D}_2,...,\mathcal{D}_n ]$, where $\mathcal{D}_j = \{ x^{(i)}, {y_w}^{(i)}, {y_l}^{(i)}, {d_j}^{(i)}\}_{i=1}^{N}$ and ${d_j}^{(i)}$ represents the i-th sample score in the dimension of $d_j$, e.g., helpfulness.

\textbf{Generation. }For generative Language Models, such as GPT~\cite{gpt42023openai,radford2018improving}, LLaMA~\cite{touvron2023llama,touvron2023llama2,llama3}, these models, i.e., $\pi_\theta$ are used to generate a sequence that approximately maximizes the following likelihood:
\begin{equation}
    \label{eq.1}
    p_\theta(y | x) = \frac{1}{|y|} \sum_{i=1}^{|y|} \log \pi_\theta(y_i | x, y_{<i})
\end{equation}

\textbf{Bradley-Terry Model. }Assuming that human preferences are generated by some latent reward models $r^*(y, x)$ under the Bradley-Terry (BT) Model~\cite{bradley1952rank}, the human preference distribution $p^*$ can be defined as:
\begin{equation}
    \label{eq.2}
    p^*(y_w \succ y_l | x) = \sigma(r^*(x, y_w) - r^*(x, y_l)).
\end{equation}
where $y_w$ and $y_l$ denote preferred and dispreferred response of same prompt $x$.

\textbf{DPO. }To eliminate explicit reward model, DPO~\cite{DPO2023Rafailov} proposes a direct optimization objective that satisfies the optimal preference policy:
\vspace{-0.2em}
\begin{equation}
\label{Eq.3}
\begin{split}
\mathcal{L}_{\text{DPO}}&(\pi_\theta; \pi_{\text{ref}})  = \\
& -\mathbb{E}_{(x, y_w, y_l) \sim \mathcal{D}} \left[ \log \sigma \left( \beta \log \frac{\pi_\theta(y_w \mid x)}{\pi_{\text{ref}}(y_w \mid x)} \right. \right. \\
& \left. \left. - \beta \log \frac{\pi_\theta(y_l \mid x)}{\pi_{\text{ref}}(y_l \mid x)} \right) \right].
\end{split}
\end{equation}

where $(x, y_w, y_l)$ denotes a preference pair consisting of the prompt, the winning response and the losing response from the preference dataset $\mathcal{D}$, $\pi_\theta$ and $\pi_{\text{ref}}$ represent the policy model and the reference model.

% CPO:
% \vspace{-0.2em}
% \begin{equation}
% \begin{split}
% \mathcal{L}(\pi_\theta;& U) = \\ & -\mathbb{E}_{(x, y_w, y_l) \sim \mathcal{D}} \biggl[ \log \sigma \biggl( \beta \log \pi_\theta(y_w \mid x) \\
% & - \beta \log \pi_\theta(y_l \mid x) \biggr) \biggr].
% \end{split}
% \end{equation}
\textbf{SimPO. }SimPO~\cite{simpo2024meng} proposes a more lightweight and easier menthod than DPO. It does not require a reference model, which uses the Eq.\eqref{eq.1} replacing the reward formulation, resulting in a new loss:
\vspace{-0.2em}
\begin{equation}
\label{Eq.4}
\begin{split}
\mathcal{L}_{\text{SimPO}}&(\pi_\theta) = \\ & -\mathbb{E}_{(x, y_w, y_l) \sim \mathcal{D}} \biggl[ \log \sigma \biggl( \frac{\beta}{|y_w|} \log \pi_\theta(y_w \mid x) \\
& \quad - \frac{\beta}{|y_l|} \log \pi_\theta(y_l \mid x) - \gamma \biggr) \biggr].
\end{split}
\end{equation}
where $\beta$ is a constant that controls the scaling of the reward difference and $\gamma$ is a target reward margin.

\textbf{MODPO. }MODPO first defines $\bm{r}^*={[{r_1}^*,...,{r_n}^*]}^T$ for multi-dimensional datasets $\bm{\mathcal{D}} = [ \mathcal{D}_1, \mathcal{D}_2,...,\mathcal{D}_n ]$. And then follows a two-stage approach: (1) margin reward modeling: Train margin reward models $\bm{r}_{\phi,-k}$ on $\mathcal{D}_{-k}$, i.e., the dimensions excluding the $k\text{-th}$ dimension. (2) Language modeling: Use a set of fixed weights $\bm{w}$ to balance different dimensions to optimizes:

\begin{equation}
\label{Eq.5}
\resizebox{0.5\textwidth}{!}{$
\begin{aligned}
&\mathcal{L}_{modpo}(\pi_{\theta_w}; r_{\phi,-k}, \pi_{sft}, \mathcal{D}_k) = \\ & - \mathbb{E}_{D_k} \left[ \log \sigma \left( \frac{\beta}{w_k} \log \frac{\pi_{\theta_w}(y_w | x)}{\pi_{sft}(y_w | x)}  - \frac{\beta}{w_k} \log \frac{\pi_{\theta_w}(y_l | x)}{\pi_{sft}(y_l | x)} \right. \right. \\
& \quad \left. \left. -  \frac{1}{W_k} W_{-k}^T r_{\phi,-k}(x, y_w) - r_{\phi,-k}(x, y_l) \right) \right]
\end{aligned}$
}
\end{equation}

==> latex/sections_article/4_RMoPO.tex <==

% \begin{figure*}[!h]
% 	\centering
% 	\includegraphics[width=0.98\textwidth]{latex/images/main/pipeline_rjq.pdf}
% 	\caption{An overview of {\ourtitle} pipeline, which consists of 2 main steps: (a) Multi-objective preference dataset preprocessed, for a prompt with two responses, i.e., $y_a$ and $y_b$, it also has three dimensions scores, e.g., helpfulness, correctness and instruction following, with the scoring criteria on the left. And for each dimension, designing a unique template makes the model focus on the current dimension to generate the answer. (b) After preprocessing dataset, we extend the raw pair $<x,y_w,y_l>$ to multiple pairs $\{(<x^*,y_w,y_l>)^i\}_{i=1}^{|d|}$. Then, we obtain every dimension weights by modeling the all tokens probabilities with Gaussian sample. Finally, we combine all dimensions with their weights into an overall $\bm{\mathcal{L}}$ to modify the policy model.  }
%     \label{fig:pipeline}
%     % \vspace{-10pt}
% \end{figure*}
\begin{figure*}[!h]
	\centering
	\includegraphics[width=0.98\textwidth]{latex/images/main/pipeline_rjq.pdf}
	\caption{The pipeline of \ourtitle~consists of two main stages: (a) \textbf{Data Preparation}: For a prompt with two responses, \( y_a \) and \( y_b \), GPT-4 scores each response based on three dimensions: helpfulness, correctness, and instruction following. For each dimension, a unique template is designed to ensure the model focuses on that specific dimension when generating the answer. (b) \textbf{Training}: A Gaussian-based adaptive weight assignment mechanism is implemented to sample the weight for each dimension. \ourtitle~is then updated using the loss function \(\bm{\mathcal{L}}\). }
    \label{fig:pipeline}
    % \vspace{-10pt}
\end{figure*}






\jqruan{see comments}
% 还是建议尽量不给读者你是拓展的谁、改写的谁、follow的谁的印象
% 这部分直接分为几个subsection，比如：
% 直敲我们的卖点：1. 怎么实现无其他模型的MO？ 2. 怎么实现adapter？

% 4.1  The Multi-Objective Derivation for~\ourtitle；
%  BT拓展那块 与 Mragin-集成回去
% 从BT到loss的详细推到步骤可以放在附录

% 4.2 Adaptive Weight Assignment 
% - (注意 alpha 与采样adapter的关联) ；

% 4.3 伪代码流程-Implementation？


% RMoPO
To take into account the diversity of human preferences and address the complexity and hardness of training multiple objectives reward models, we propose Adaptive Multi-objective Preference Optimization without
Rewards and References (\ourtitle), a more lightweight and efficient preference optimization method. In addition, we raise a weight assignment strategy based on Gaussian sampling in the generative spatial probability, which enables the Language Models to adaptively adjust the weight assignments among multiple dimensions during training rather than assigning fixed weights. The complete pipeline of our method is illustrated in Figure \ref{fig:pipeline}.

\subsection{The Multi-Objective Derivation for~\ourtitle}
\textbf{Multi-Objective BT Model. }Traditional BT model fuses the all dimensions reward scores into one $r(x,y)$, which will disregard the inherent significance of each dimension. To tackle this, we can extend the Eq.\eqref{eq.2} to multiple dimensions as following:
\begin{equation}
    \label{eq.6}
    \begin{split}
    P(y_w \succ &\,y_l\,|\,x;\,\bm\alpha;\,\bm{d}) = \\
    &\prod\limits_{i=1}^{|\bm\alpha|} {\left[ \sigma^{\alpha_i}(\bm{r}(x^{*}, y_w) - \bm{r}(x^{*}, y_l)) \right]} \\
    &\text{s.t.}\: \sum_{i=1}^{|\bm\alpha|} \alpha_i = 1,\: x^{*} = f(x, \bm{d}) 
    \end{split}
\end{equation}
where $\bm\alpha = [\alpha_1,...,\alpha_n]$ represents different dimension weights, and $f(x|\bm{d})$ restructure x accordingly in different dimensions. It is not hard to find that the multi-objective BT Model will degrade to traditional BT Model (Eq.\eqref{eq.2}), when $|\bm{d}|=1$, i.e., the basic preference optimization.

\textbf{{\ourtitle}  objective. }Finally, we can obtain $\bm\alpha=[\alpha_1,...,\alpha_n]$, representing multi-dimensional weights. To learn the relativity among different dimensions, we normalize all the weights as following:
\begin{equation}
    \label{Eq.7}
    \alpha_i = \frac{e^{\alpha_i}}{\sum_{j=1}^{n} e^{\alpha_j}}.
\end{equation}
And then we obtain the {\ourtitle} objective by combining Eq.\eqref{eq.1}, Eq.\eqref{Eq.4} and Eq.\eqref{eq.6}:
\begin{equation}
\label{Eq.ours}
    \begin{split}
        \mathcal{L}_{\text{\ourtitle}}&(\pi_\theta; \bm{\alpha}; \bm{d}) = 
        - \mathbb{E}_{(x, y_w, y_l)\sim \mathcal{D}} \\ & \biggl[ \sum_{i=1}^{|\bm\alpha|} \alpha_i \log \sigma \biggl(\frac{\beta}{|{y_w}|} \log \pi_\theta({y_w} \mid x^{*}) \\
        & \quad - \frac{\beta}{|{y_l}|} \log \pi_\theta({y_l} \mid x^{*}) ) \biggr].\\
        & \text{s.t.}\; x^{*}=f(x|\bm{d}) 
    \end{split}
\end{equation}
where for a triple $<x,y_w,y_l>$ and multi-dimension $\bm{d}$, uses a map function $f(x)$, e.g., a prompt template as $f$, to generate $x^{*}={\{x_i,y_w,y_l \}}_{i=1}^{|\bm{d}|}$ for representing probability distribution in different dimension.
% \subsection{Methodology}
% \textbf{Reward margins. } Following SimPO~\cite{simpo2024meng}, we add a target reward margin for each dimension, $\bm\gamma > 0$ to Eq.\eqref{eq.6} to ensure that each dimension reward for the winning response exceeds the losing response by at least $\bm\gamma$:
% \begin{equation}
%     \label{eq.7}
%     \begin{split}
%     P(y_w \succ &\,y_l\,|\,x;\,\bm\alpha;\,\bm{d}) = \\
%     &\prod\limits_{i=1}^{|\bm\alpha|} {\left[ \sigma^{\alpha_i}(r(x^{*}, y_w) - r(x^{*}, y_l) - \gamma) \right]} \\
%     &s.t.\: \sum_{i=1}^{|\bm\alpha|} \alpha_i = 1,\: x^{*} = f(x|\bm{d}) 
%     \end{split}
% \end{equation}
% Compared to increasing the margin in the overall result, augmenting the margin in each dimension individually can enhance the model's performance in each specific dimension.
\subsection{Adaptive Weight Assignment}
\textbf{Gaussian-sample weight assignment. } To enable LMs to dynamically allocate multi-dimensional weights during training, we model the sequential and auto-regressive generation for LMs. 
As Eq.\eqref{eq.1} shown, the generation of these responses occurs in a token level. 
For each dimension response, we catch all tokens with their probabilities of response, considering that response consists of $T$ tokens of $y=y^{<T+1}:{\{<t_i,p_i>\}}_{i=1}^{T}$ where $<t_s,p_s>$ represents the $s\text{-th}$ token and its probability, respectively. 
Given a prompt $x$ and first $T-1$ tokens of the response $y^{<T}$, the LMs predicts the probability distribution of the next token $\pi_\theta(\cdot|x;\,y^{<T})$. 
Based on next-token prediction theory~\cite{shannon1948mathematical, Maximum1983Bahl}, the higher the probability of a token, the greater the likelihood that the LMs will generate the current token. 
Similarly, the probability of tokens can also reflect the significance of the current dimension.
Therefore, we introduce this into weight assignment:
\begin{equation}
    \label{Eq.9}
    \begin{aligned}
    &\alpha \sim \mathcal{N}(\mu, \sigma^2), \\
    \text{s.t.} \quad \mu  = \frac{1}{|T|} &\sum_{i=1}^{|T|}\; p_i;  \hspace{0.2em}\sigma^2 = \frac{1}{|T|} \sum_{i=1}^{|T|} (p_i - \mu)^2
\end{aligned}
\end{equation}
where $\alpha$ reflects the probability distribution over the current output space of LMs. We use the different $\alpha$ to assign weights for multiple dimensions by the distinctive probability distribution.

\subsection{Implementation details}

% As shown in Figure \ref{fig:pipeline}, {\ourtitle} takes the multi-objective training progress into two stages. 
% \textbf{Firstly}, we extend the original prompt to diversity prompts for mapping each dimension.
% We provide a set of universal templates to adapt to different dimensions, which makes LMs focus on a specific dimension when answering questions.
% And one obvious benefit is that for a specific prompt and its response, we can obtain diversity probability distribution through our method.
% \textbf{Regarding the second phase}, we transfer
{\ourtitle} transfers an original quadruple $<x,y_w,y_l,\bm{d}>$ into a set of quadruples $\{<x,y_w,y_l,d_i>\}_{i=1}^{|\bm{d}|}$. And then we design a map function $f$, which changes $x$ according to different dimensions, i.e., $x_i^* = f(x|d_i)$. Subsequently, we concatenate the multi-dimensional prompts $x_i^*$ with the winning response $y_w$ and the losing response $y_l$ individually as inputs to the policy model $\pi_\theta$. 
We can easily obtain the all tokens probabilities $p_i^w$ of the winning responses and $p_i^l$ of the losing responses. Then, we add both responses tokens probabilities, i.e., $p_i=p_i^w+p_i^l$, in which $p_i$ means the policy model confidence in the $d_i$ dimension.
Based on these tokens probabilities, we model $p_i$ by Gaussian Sample. And sample a probability $\alpha_i$ as the weight for the $d_i$ dimension.
In addition, we utilize the LM generation metric to obtain the loss between the winning and losing response, which can be formulated as $l=\log\sigma(\frac{\beta}{|{y_w}|} \log \pi_\theta({y_w} \mid x^{*})-\frac{\beta}{|{y_l}|} \log \pi_\theta({y_l} \mid x^{*}))$.
Taking into account the effect of weight $\alpha_i$, we finally obtain the loss $l=\alpha_i\log\sigma(\frac{\beta}{|{y_w}|} \log \pi_\theta({y_w} \mid x_i^{*})-\frac{\beta}{|{y_l}|} \log \pi_\theta({y_l} \mid x_i^{*}))$ in the dimension of $d_i$.
We provide the pseudocode in Algorithm \ref{alg:amopo} in details.
